BayesMortalityPlus: A package in R for Bayesian graduation of mortality modelling

The BayesMortalityPlus package provides a framework for modelling and predicting mortality data. The package includes tools for the construction of life tables based on Heligman-Pollard laws, and also on dynamic linear smoothers. Flexibility is available in terms of modelling so that the response variable may be modeled as Poisson, Binomial or Gaussian. If temporal data is available, the package provides a Bayesian implementation for the well-known Lee-Carter model that allows for estimation, projection of mortality over time, and assessment of uncertainty of any linear or nonlinear function of parameters such as life expectancy. Illustrations are considered to show the capability of the proposed package to model mortality data.

==> BMP <==
\begin{thebibliography}{44}
\newcommand{\enquote}[1]{``#1''}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi:\discretionary{}{}{}#1}\else
  \providecommand{\doi}{doi:\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem[{Banerjee \emph{et~al.}(2004)Banerjee, Carlin, and
  Gelfand}]{gelfand04}
Banerjee S, Carlin BP, Gelfand AE (2004).
\newblock \emph{Hierarchical Modeling and Analysis for Spatial Data}.
\newblock Monographs on Statistics and Applied Probability 101, 1 edition.
  Chapman \& Hall/CRC.

\bibitem[{Barigou and Goffard(2022)}]{stanmomo}
Barigou K, Goffard PO (2022).
\newblock \emph{StanMoMo: Bayesian Mortality Modelling with 'Stan'}.
\newblock R package version 1.1.0,
  \urlprefix\url{https://CRAN.R-project.org/package=StanMoMo}.

\bibitem[{Booth \emph{et~al.}(2002)Booth, Maindonald, and Smith}]{Booth2002}
Booth H, Maindonald JH, Smith L (2002).
\newblock \enquote{Applying Lee-Carter under conditions of variable mortality
  decline.}
\newblock \emph{Population Studies}, \textbf{56}, 325 -- 336.

\bibitem[{Bowers(1986)}]{bowers1986actuarial}
Bowers N (1986).
\newblock \emph{Actuarial Mathematics}.
\newblock 1 edition. Society of Actuaries.
\newblock ISBN 9780938959106.
\newblock \urlprefix\url{https://books.google.com.br/books?id=jrjuAAAAMAAJ}.

\bibitem[{Camarda(2012)}]{mortsmooth}
Camarda CG (2012).
\newblock \enquote{{MortalitySmooth}: An {R} Package for Smoothing {P}oisson
  Counts with {P}-Splines.}
\newblock \emph{Journal of Statistical Software}, \textbf{50}(1), 1--24.
\newblock \urlprefix\url{http://www.jstatsoft.org/v50/i01/}.

\bibitem[{Camarda(2019)}]{Carmada2019}
Camarda CG (2019).
\newblock \enquote{{Smooth constrained mortality forecasting}.}
\newblock \emph{Demographic Research}, \textbf{41}(38), 1091--1130.
\newblock \doi{10.4054/DemRes.2019.41.38}.
\newblock
  \urlprefix\url{https://ideas.repec.org/a/dem/demres/v41y2019i38.html}.

\bibitem[{Camarda \emph{et~al.}(2016)Camarda, Eilers, and Gampe}]{Carmada2016}
Camarda CG, Eilers PH, Gampe J (2016).
\newblock \enquote{Sums of smooth exponentials to decompose complex series of
  counts.}
\newblock \emph{Statistical Modelling}, \textbf{16}(4), 279--296.
\newblock \doi{10.1177/1471082X16641796}.
\newblock \urlprefix\url{https://doi.org/10.1177/1471082X16641796}.

\bibitem[{Carlin(1992)}]{Carlin1992}
Carlin BP (1992).
\newblock \enquote{A simple Monte Carlo approach to Bayesian graduation.}
\newblock In \emph{Transactions of the Society of Actuaries}. Citeseer.

\bibitem[{Carter and Kohn(1994)}]{Carter1994}
Carter C, Kohn R (1994).
\newblock \enquote{On Gibbs sampling for state space models.}
\newblock \emph{Biometrika}, \textbf{81}(3), 541–553.

\bibitem[{Currie \emph{et~al.}(2004)Currie, Durban, and Eilers}]{Eilers2004}
Currie ID, Durban M, Eilers PH (2004).
\newblock \enquote{Smoothing and forecasting mortality rates.}
\newblock \emph{Statistical Modelling}, \textbf{4}(4), 279--298.
\newblock \doi{10.1191/1471082X04st080oa}.
\newblock \urlprefix\url{https://doi.org/10.1191/1471082X04st080oa}.

\bibitem[{Czado \emph{et~al.}(2005)Czado, Delwarde, and Denuit}]{Czado2005}
Czado C, Delwarde A, Denuit M (2005).
\newblock \enquote{Bayesian Poisson log-bilinear mortality projections.}
\newblock \emph{Insurance: Mathematics and Economics}, \textbf{36}(3),
  260--284.
\newblock ISSN 0167-6687.
\newblock \doi{https://doi.org/10.1016/j.insmatheco.2005.01.001}.
\newblock
  \urlprefix\url{https://www.sciencedirect.com/science/article/pii/S0167668705000302}.

\bibitem[{Dellaportas \emph{et~al.}(2001)Dellaportas, Smith, and
  Stavropoulos}]{dellaportas2001bayesian}
Dellaportas P, Smith AF, Stavropoulos P (2001).
\newblock \enquote{Bayesian analysis of mortality data.}
\newblock \emph{Journal of the Royal Statistical Society: Series A (Statistics
  in Society)}, \textbf{164}(2), 275--291.

\bibitem[{Dodd \emph{et~al.}(2018)Dodd, Forster, Bijak, and
  Smith}]{Forster2018}
Dodd E, Forster J, Bijak J, Smith P (2018).
\newblock \enquote{Smoothing mortality data: the English life table, 2010-12.}
\newblock \emph{Journal of the Royal Statistical Society: Series A (Statistics
  in Society)}, \textbf{181}(3), 717--735.

\bibitem[{Frühwirth-Schnatter(1994)}]{Sylvia1994}
Frühwirth-Schnatter S (1994).
\newblock \enquote{DATA AUGMENTATION AND DYNAMIC LINEAR MODELS.}
\newblock \emph{Journal of Time Series Analysis}, \textbf{15}(2), 183--202.
\newblock \doi{10.1111/j.1467-9892.1994.tb00184.x}.

\bibitem[{Gamerman and Lopes(2006)}]{gamerman}
Gamerman D, Lopes H (2006).
\newblock \emph{Markov Chain Monte Carlo: Stochastic Simulation for Bayesian
  Inference}.
\newblock Texts in Statistical Science, 2 edition. Taylor \& Francis.

\bibitem[{Gavrilov and Gavrilova(2011)}]{gavrilov2011mortality}
Gavrilov LA, Gavrilova NS (2011).
\newblock \enquote{Mortality measurement at advanced ages: a study of the
  Social Security Administration Death Master File.}
\newblock \emph{North American actuarial journal}, \textbf{15}(3), 432--447.

\bibitem[{Gompertz(1825)}]{gompertz1825xxiv}
Gompertz B (1825).
\newblock \enquote{XXIV. On the nature of the function expressive of the law of
  human mortality, and on a new mode of determining the value of life
  contingencies. In a letter to Francis Baily, Esq. FRS \&c.}
\newblock \emph{Philosophical transactions of the Royal Society of London},
  \textbf{115}, 513--583.

\bibitem[{Heligman and Pollard(1980)}]{heligman1980age}
Heligman L, Pollard JH (1980).
\newblock \enquote{The age pattern of mortality.}
\newblock \emph{Journal of the Institute of Actuaries}, \textbf{107}(1),
  49--80.

\bibitem[{Hilton \emph{et~al.}(2019)Hilton, Dodd, Forster, and
  Smith}]{HiltonForster2019}
Hilton J, Dodd E, Forster JJ, Smith PW (2019).
\newblock \enquote{Projecting UK mortality by using Bayesian generalized
  additive models.}
\newblock \emph{Journal of the Royal Statistical Society, Series C (Applied
  Statistics)}, \textbf{68}(1), 29--49.

\bibitem[{HMD(2022)}]{hmd}
HMD (2022).
\newblock \enquote{Human Mortality Database. Max Planck Institute for
  Demographic Research (Germany), University of California, Berkeley (USA), and
  French Institute for Demographic Studies (France).}
\newblock \url{https://www.mortality.org/}.
\newblock Accessed: 2022-07-28.

\bibitem[{Hustead(2005)}]{hustead2005ending}
Hustead EC (2005).
\newblock \enquote{Ending the mortality table.}
\newblock In \emph{Living to 100 and Beyond Symposium}.

\bibitem[{Hyndman and {Shahid Ullah}(2007)}]{Hydman2007}
Hyndman RJ, {Shahid Ullah} M (2007).
\newblock \enquote{Robust forecasting of mortality and fertility rates: A
  functional data approach.}
\newblock \emph{Computational Statistics \& Data Analysis}, \textbf{51}(10),
  4942--4956.
\newblock ISSN 0167-9473.
\newblock \doi{https://doi.org/10.1016/j.csda.2006.07.028}.

\bibitem[{Kimeldorf and Jones(1967)}]{Kimeldorf1967}
Kimeldorf G, Jones DA (1967).
\newblock \enquote{Bayesian graduation.}
\newblock \emph{Transactions of the Society of Actuaries}, \textbf{19}(54 part
  1), 66--112.

\bibitem[{Lai(2012)}]{lai2012human}
Lai C (2012).
\newblock \enquote{Human mortality curves that decelerate to a plateau.}
\newblock \emph{Mathematical and Computer Modelling}, \textbf{55}(3-4),
  1118--1128.

\bibitem[{Lee and Carter(1992)}]{Lee1992}
Lee R, Carter L (1992).
\newblock \enquote{Modeling and forecasting U.S. mortality.}
\newblock \emph{Journal of the American Statistical Association},
  \textbf{87}(419), 659--671.
\newblock \doi{10.2307/2290201}.

\bibitem[{Lee and Miller(2001)}]{LeeMiller2001}
Lee R, Miller T (2001).
\newblock \enquote{Evaluating the performance of the Lee-Carter method for
  forecasting mortality.}
\newblock \emph{Demography}, \textbf{38}, 537--549.
\newblock \doi{10.2307/3088317}.

\bibitem[{Li(2013)}]{Li2013}
Li J (2013).
\newblock \enquote{{A Poisson common factor model for projecting mortality and
  life expectancy jointly for females and males}.}
\newblock \emph{Population Studies}, \textbf{67}(1), 111--126.
\newblock \doi{10.1080/00324728.2012.689}.

\bibitem[{Li \emph{et~al.}(2004)Li, Lee, and Tuljapurkar}]{LiLee04}
Li N, Lee RD, Tuljapurkar S (2004).
\newblock \enquote{Using the Lee–Carter method to forecast mortality for
  populations with limited data.}
\newblock \emph{International Statistical Review}, \textbf{72}, 19--36.

\bibitem[{Neves and Migon(2007)}]{MigonNeves2007}
Neves C, Migon HS (2007).
\newblock \enquote{Bayesian graduation of mortality rates: An application to
  reserve evaluation.}
\newblock \emph{Insurance: Mathematics and Economics}, \textbf{40}, 424–434.

\bibitem[{Pascariu(2022)}]{mortlaws}
Pascariu MD (2022).
\newblock \emph{MortalityLaws: Parametric Mortality Models, Life Tables and
  HMD}.
\newblock R package version 1.9.3,
  \urlprefix\url{https://CRAN.R-project.org/package=MortalityLaws}.

\bibitem[{Pedroza(2006)}]{Pedroza2006}
Pedroza C (2006).
\newblock \enquote{{A Bayesian forecasting model: predicting U.S. male
  mortality}.}
\newblock \emph{Biostatistics}, \textbf{7}(4), 530--550.
\newblock ISSN 1465-4644.
\newblock \doi{10.1093/biostatistics/kxj024}.
\newblock
  \eprint{https://academic.oup.com/biostatistics/article-pdf/7/4/530/610324/kxj024.pdf},
  \urlprefix\url{https://doi.org/10.1093/biostatistics/kxj024}.

\bibitem[{Petris \emph{et~al.}(2009)Petris, Petrone, and
  Campagnoli}]{petris2009dynamic}
Petris G, Petrone S, Campagnoli P (2009).
\newblock \enquote{Dynamic linear models.}
\newblock In \emph{Dynamic linear models with R}, pp. 31--84. Springer.

\bibitem[{{R Core Team}(2020)}]{RCoreTeam}
{R Core Team} (2020).
\newblock \emph{R: A Language and Environment for Statistical Computing}.
\newblock R Foundation for Statistical Computing, Vienna, Austria.
\newblock \urlprefix\url{https://www.R-project.org/}.

\bibitem[{Renshaw \emph{et~al.}(1996)Renshaw, Haberman, and
  Hatzopoulos}]{Renshaw1996}
Renshaw A, Haberman S, Hatzopoulos P (1996).
\newblock \enquote{The Modeling of Recent Mortality Trends in United Kingdom
  Male Assured Lives.}
\newblock \emph{British Actuarial Journal}, \textbf{2}.
\newblock \doi{10.1017/S1357321700003470}.

\bibitem[{Rob J~Hyndman \emph{et~al.}(2019)Rob J~Hyndman, Tickle, and
  Maindonald.}]{demography}
Rob J~Hyndman wcfHB, Tickle L, Maindonald J (2019).
\newblock \emph{demography: Forecasting Mortality, Fertility, Migration and
  Population Data}.
\newblock R package version 1.22,
  \urlprefix\url{https://CRAN.R-project.org/package=demography}.

\bibitem[{Sharrow(2012)}]{HPbayes}
Sharrow DJ (2012).
\newblock \emph{HPbayes: Heligman Pollard mortality model parameter estimation
  using Bayesian Melding with Incremental Mixture Importance Sampling}.
\newblock R package version 0.1,
  \urlprefix\url{https://CRAN.R-project.org/package=HPbayes}.

\bibitem[{Sherris and Njenga(2011)}]{Njenga2011}
Sherris M, Njenga C (2011).
\newblock \enquote{Modeling mortality with a Bayesian vector autoregression.}
\newblock \emph{Technical report}, Research Paper 2011ACTL04. Australian School
  of Business, University of New South Wales, Sydney.

\bibitem[{{Stan Development Team}(2020)}]{rstan}
{Stan Development Team} (2020).
\newblock \enquote{{{RStan}}: the {R} interface to {Stan}.}
\newblock \urlprefix\url{http://mc-stan.org/}.

\bibitem[{Tang \emph{et~al.}(2021)Tang, Dodd, and Forster}]{Forster2021}
Tang K, Dodd E, Forster J (2021).
\newblock \enquote{Joint modelling of male and female mortality rates using
  adaptive P-splines.}
\newblock \emph{Annals of Actuarial Science}, \textbf{16}, 1--17.
\newblock \doi{10.1017/S1748499521000105}.

\bibitem[{Turner and Firth(2022)}]{gnm}
Turner H, Firth D (2022).
\newblock \emph{Generalized nonlinear models in R: An overview of the gnm
  package}.
\newblock R package version 1.1-2,
  \urlprefix\url{https://cran.r-project.org/package=gnm}.

\bibitem[{Villegas \emph{et~al.}(2018)Villegas, Kaishev, and
  Millossovich}]{stmomo}
Villegas AM, Kaishev VK, Millossovich P (2018).
\newblock \enquote{{StMoMo}: An {R} Package for Stochastic Mortality Modeling.}
\newblock \emph{Journal of Statistical Software}, \textbf{84}(3), 1--38.
\newblock \doi{10.18637/jss.v084.i03}.

\bibitem[{West and Harrison(1997)}]{West97}
West M, Harrison J (1997).
\newblock \emph{Bayesian forecasting and dynamic models.}
\newblock 2 edition. Springer.

\bibitem[{Wickham \emph{et~al.}(2022)Wickham, François, Henry, and
  Müller}]{dplyr}
Wickham H, François R, Henry L, Müller K (2022).
\newblock \emph{dplyr: A Grammar of Data Manipulation}.
\newblock R package version 1.0.9,
  \urlprefix\url{https://CRAN.R-project.org/package=dplyr}.

\bibitem[{Wood(2006)}]{Wood2006}
Wood SN (2006).
\newblock \emph{Generalised Additive Models: an Introduction with R}.
\newblock 1 edition. Boca Raton: Chapman and Hall– CRC.

\end{thebibliography}

